The hydrophobic effect characterises the thermodynamic signature of amyloid fibril growth

Many proteins have the potential to aggregate into amyloid fibrils, which are associated with a wide range of human disorders including Alzheimer's and Parkinson's disease. In contrast to that of folded proteins, the thermodynamic stability of amyloid fibrils is not well understood: specifically the balance between entropic and enthalpic terms, including the chain entropy and the hydrophobic effect, are poorly characterised. Using simulations of a coarse-grained protein model we delineate the enthalpic and entropic contributions dominating amyloid fibril elongation, predicting a characteristic temperature-dependent enthalpic signature. We confirm this thermodynamic signature by performing calorimetric experiments and a meta-analysis over published data. From these results, we can also elucidate the necessary conditions to observe cold denaturation of amyloid fibrils. Overall, we show that amyloid fibril elongation is associated with a negative heat capacity, the magnitude of which correlates closely with the hydrophobic surface area that is buried upon fibril formation, highlighting the importance of hydrophobicity for fibril stability.

==> abstract_long.tex <==
\begin{abstract}
    The hydrophobic effect is the main driver of protein folding. Under certain conditions, stretches of hydrophobic amino acids can lead to the aggregation of proteins into $\beta$-strand-dominated amyloid fibrils associated with several degenerative diseases. Amyloid fibrils are thermodynamically highly stable, but the molecular origin of the stability is not well understood. While amyloid fibrils usually dissociate at very high temperatures, some fibrils also dissociate close to 0$^{\circ}$C, reminiscent of cold denaturation of proteins. Here, we introduce a consistent treatment of the temperature-dependent hydrophobicity in a coarse-grained lattice model to describe the elongation of a preformed amyloid fibril at different temperatures. With this model, we show that cold denaturation only occurs when (1) the hydrophobic effect represents a significant component of the fibril stability, (2) the overall stability of the fibril is sufficiently low and (3) fibril elongation changes from being an endothermic reaction at lower temperatures to an exothermic reaction at higher temperatures. Furthermore, we show that in addition to the hydrophobic effect, the backbone entropy has a significant influence on the fibril stability. Finally, the model shows that fibril formation typically is an exothermic process, with a negative differential heat capacity for elongation with both characteristics originating from the hydrophobic effect. The predictions by our model are confirmed by the available experimental data from the literature and our own experiments. Taken together, this work presents a comprehensive experimental, theoretical and computational analysis of the dominating role of hydrophobicity in the thermodynamic characteristics of amyloid fibrils.
\end{abstract}

==> abstract_short.tex <==
\begin{abstract}
Many proteins have the potential to aggregate into amyloid fibrils, which are associated with a wide range of human disorders including Alzheimer’s and Parkinson’s disease. In contrast to that of folded proteins, the thermodynamic stability of amyloid fibrils is not well understood: specifically the balance between entropic and enthalpic contributions, including the chain entropy and the hydrophobic effect, are poorly characterised. Here we use simulations that can capture these contributions explicitly. We also perform calorimetric experiments at different temperatures and gather published data to investigate the enthalpic signature of fibril growth. From our results, we elucidate the necessary conditions to observe cold denaturation in amyloid fibrils. The hydrophobic term in our model can explain why amyloid fibril elongation is generally associated with a negative heat capacity. Moreover, the magnitude of this heat capacity correlates closely with the hydrophobic surface area that is buried upon fibril formation.
\end{abstract}
